Formation and Optimisation of Vein Networks in Physarum

Physarum polycephalum is an acellular slime mould that grows as a highly adaptive network of veins filled with protoplasm. As it forages, Physarum dynamically rearranges its network structure as a response to local stimuli information, optimising the connection between food sources. This high-level behaviour was already exploited to solve numerous optimisation problems. We develop a flow-based model for the adaptive network formation of Physarum, which solves some inconsistencies of previous models. We first derive a general class of equations describing the adaptation and flow dynamics of a static network comprised of elastic channels filled with an incompressible fluid undergoing a Hagen-Poiseuille flow. An explicit form of the model is obtained by minimising the total power dissipated by the network. Considering a more general functional form of the adaptive equations, a phase transition in the system is also found. The model is used for maze-solving and to build efficient and resilient networks in an arena mimicking mainland Portugal. By comparing the resulting networks with the real Portuguese railway system, we found that the model produced networks with a better overall performance when considering fluctuations in the network flows. Finally, the adaption model is extended to incorporate the network growth in the presence of multiple food sources. The coupling of both processes produces networks with similar traits to several network systems found in nature. We found that when the food sources operate alternately, the model can replicate the direct connections between the food sources observed in Physarum.

==> settings.tex <==
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{hyphenat}
\usepackage{graphicx}
\usepackage{newfloat}
\DeclareFloatingEnvironment[name={Gráfico}]{graph}

\usepackage{subcaption}
\DeclareCaptionSubType{graph}
\usepackage{amsmath,amssymb,cancel,breqn}
\usepackage{lipsum}
\usepackage{bm}
\usepackage{float}
\usepackage[usenames,dvipsnames]{color}
\usepackage{multirow} %
\usepackage{bigstrut}
\usepackage{xfrac}
\usepackage{wasysym}
\usepackage{afterpage}

\usepackage{siunitx}
\sisetup{separate-uncertainty = true}


\usepackage{mathtools}



\usepackage[english]{todonotes}

\newcommand{\victor}[1]{{\color{orange}V: #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}
\newcommand{\red}[1]{{\color{red} #1}}

\newcommand{\todov}[1]{\todo[inline, author=V, color= orange]{#1}}
\newcommand{\todog}[1]{\todo[inline, author=G, color= magenta]{#1}}
\newcommand{\todok}[1]{\todo[inline, author=K, color= cyan]{#1}}

\usepackage{color,soul}

\setul{0.5ex}{0.3ex}
\setulcolor{red}

\usepackage{placeins}

\usepackage{fancyhdr}
\pagestyle{plain}

\makeatletter
\def\Dated@name{}
\makeatother

\usepackage{textcomp}

\renewcommand{\thetable}{\arabic{table}}

\graphicspath{{./pics/}}
\usepackage{verbatim}




\usepackage{gensymb}
\usepackage{multicol}
\usepackage{physics}
\usepackage{empheq}
\usepackage[theorems,skins]{tcolorbox}
\newtcolorbox{mymathbox}[1][]{colback=white, sharp corners, #1}
\usepackage{siunitx}
\sisetup{inter-unit-product =$\cdot$}
\usepackage{bigints}
\usepackage{pifont}
\usepackage{amssymb}

\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt
                     \hbox{.}\hbox{.}}}%
                     =}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\NewDocumentCommand{\evalat}{sO{\big}mm}{%
  \IfBooleanTF{#1}
   {\mleft. #3 \mright|_{#4}}
   {#3#2|_{#4}}%
}

\newcommand{\ep}{\varepsilon}


\usepackage{wrapfig}

\newcommand{\ra}{$\rightarrow \ $}
\newcommand{\Ra}{$\Rightarrow{}$}

\newcommand\Warning{%
 \makebox[2 em][c]{%
 \makebox[0pt][c]{\raisebox{.2em}{\small!}}%
 \makebox[0pt][c]{\color{red}\LARGE$\bigtriangleup$}}}%

\newcommand{\mb}[1]{\mathbf{#1}}

\newcommand{\fb}[1]{\framebox{\blue{#1}}}

\newcommand{\rb}[1]{\textbf{\red{#1}}}

\newcommand{\bb}[1]{\textbf{\blue{#1}}}

\newcommand{\gb}[1]{\textbf{\textcolor{OliveGreen}{#1}}}


\newenvironment{nalign}{
    \begin{equation}
    \begin{aligned}
}{
    \end{aligned}
    \end{equation}
    \ignorespacesafterend
}


\newcommand{\E}{\mathcal{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\eq}{\Leftrightarrow}

\newcommand{\avg}[1]{\left< #1 \right>}


